QACE: Asking Questions to Evaluate an Image Caption

In this paper, we propose QACE, a new metric based on Question Answering for Caption Evaluation. QACE generates questions on the evaluated caption and checks its content by asking the questions on either the reference caption or the source image. We first develop QACE-Ref that compares the answers of the evaluated caption to its reference, and report competitive results with the state-of-the-art metrics. To go further, we propose QACE-Img, which asks the questions directly on the image, instead of reference. A Visual-QA system is necessary for QACE-Img. Unfortunately, the standard VQA models are framed as a classification among only a few thousand categories. Instead, we propose Visual-T5, an abstractive VQA system. The resulting metric, QACE-Img is multi-modal, reference-less, and explainable. Our experiments show that QACE-Img compares favorably w.r.t. other reference-less metrics. We will release the pre-trained models to compute QACE.

==> rsc/table_ablation_answer_similarity.tex <==
\begin{table}[!t]
\centering 
\small
\begin{tabular}{lccc}
\toprule
                  & Pascal50s  & Composite     & Flickr8k \\
\midrule
VisQuest-Ref-F1   & 75.1       & 49.3 & 40.5 \\ 
VisQuest-Ref-BS   & 75.1       & 49.3 & 40.5 \\
\midrule
VisQuest-Img-F1      & 70.0   & 19.1 & 28.9- \\
VisQuest-Img-BS      & 70.0   & 19.1 & 28.9- \\
\bottomrule
\end{tabular}
\caption{Ablation studies on answer similarity function. BS denotes BERTScore. All p-values in the results are $<$ 0.05. % To be checked 
}

\label{table_ablation_answer_similarity}
\end{table}

